SoK: When FL Clients Cannot Train -- Delegated Federated Learning for IoT

Federated learning (FL) assumes that a client can perform the computation required to produce its own contribution. This assumption is often unrealistic for resource-constrained Internet of Things (IoT) devices, motivating designs that delegate some or all client-side training to more capable parties. We systematize this setting as delegated federated learning (Delegated FL), where data ownership and execution of owner-attributed learning are separated. We develop a framework that examines three dimensions over the same delegated transition: delegate-view privacy, delegated attribution, and constrained-owner feasibility. Our audit of 29 systems reveals a recurring composition gap. Privacy mechanisms protect selected artifacts without necessarily characterizing the accumulated view. Attribution mechanisms establish individual execution relations without necessarily binding the complete delegated transition. Furthermore, computational offloading does not establish whether the remaining workload fits the owner's resource budget. Two controlled studies on Raspberry Pi devices illustrate these gaps. We show that encrypted inputs can coexist with information leakage through an exposed residual and that locally retained labels remain inferable from split-learning gradients. We also show that message authentication can reject tampering without establishing that the executor performed the prescribed computation. Our findings demonstrate why individually established guarantees do not necessarily support the same end-to-end claim and motivate evaluating privacy, attribution, and residual owner cost over the same delegated transition.

==> 00_Abstract.tex <==
\begin{abstract}
Federated learning (FL) assumes that a client can perform the computation required to produce its own contribution. This assumption is often unrealistic for resource-constrained Internet of Things (IoT) devices, motivating designs that delegate some or all client-side training to gateways, edge nodes, peers, or cloud services. We systematize this setting as delegated federated learning (Delegated FL), where data ownership and execution of owner-attributed learning are separated. We analyze Delegated FL along three coupled dimensions: delegate-view privacy, which concerns what an executor or coalition can infer from its accumulated observations; delegated attribution, which concerns how owner authorization, input, state, prescribed work, executor, result, and admission are bound; and constrained-owner feasibility, which concerns the complete learning and assurance workload that remains with the owner. Our corpus audit reveals a recurring composition gap: privacy mechanisms protect selected artifacts without necessarily characterizing the accumulated view, integrity mechanisms establish selected relations without necessarily binding the complete delegated transition, and computational offloading does not by itself establish feasibility for a constrained owner. Two controlled studies illustrate these gaps at the owner--executor boundary: protected inputs can coexist with direct leakage through an exposed intermediate, locally retained labels remain inferable from split-learning boundary artifacts, and message authentication can reject tampering without establishing that an authorized executor performed the prescribed computation. These findings motivate evaluating privacy, delegated attribution, and residual owner cost over the same delegated transition rather than treating them as independent properties.
\end{abstract}
